Domain-Invariant Representation Learning from EEG with Private Encoders

Deep learning based electroencephalography (EEG) signal processing methods are known to suffer from poor test-time generalization due to the changes in data distribution. This becomes a more challenging problem when privacy-preserving representation learning is of interest such as in clinical settings. To that end, we propose a multi-source learning architecture where we extract domain-invariant representations from dataset-specific private encoders. Our model utilizes a maximum-mean-discrepancy (MMD) based domain alignment approach to impose domain-invariance for encoded representations, which outperforms state-of-the-art approaches in EEG-based emotion classification. Furthermore, representations learned in our pipeline preserve domain privacy as dataset-specific private encoding alleviates the need for conventional, centralized EEG-based deep neural network training approaches with shared parameters.

==> Outline.tex <==
\section*{Outline}
A fundamental problem of Deep Learning approaches is the lack of generalization capability to new data. Therefore, transfer learning methods are often used to apply a trained model to new data. However, transfer learning methods are laborious and suffer from problems such as catastrophic forgetting. We propose a new learning paradigm, multi-source learning. Thereby, we train a model to solve a task in different domains, i.e. on different datasets, simultaneously. To prevent overfitting on a subset of the data, we learn domain-invariant representations of the data using aligned private encoders. By using such representations, it is possible to combine different small data sets into one large data set, increase privacy, and increase the signal-to-noise ratio of the representation. We demonstrate that using our multi-source learning approach, it is possible to reduce the domain variance of the learned representations, while the performance in the learned task is only slightly behind that of a standard single-source model. We also highlight multi-source specific problems to be addressed in the future.
\\
\\
%1. What is the problem?
%- multi-source learning in general
%- more specific in context of EEG data
% this is not a problem per-se yet:
Many models and methods for emotion recognition based on EEG have been proposed, most of them worked well only in the scenario that the training and test data were from the same distribution or domain i.e. coming from one participant. However, such learning models fail to recognize emotions across domains due to the distribution mismatch of EEG features. Learning models that extract emotions across subjects have been proposed, however, learning across EEG datasets has not been proposed yet. 

%2. What do we gain by solving the problem?
a model, that is capable of solving a Task across multiple domains. Such a multi-source learning approach allow to combine multiple small datasets for training a model. This omits the need of large therefore expensive datasets. In a addition, a model that uses domain-invariant features can increase the privacy as it gets harder to conclude from which data-source, \textit{e.g.} from which participant, a sample was drawn. Furthermore the adaption of such a model towards data of a new data-source gets very simple.
This has not been done in the past due to the challenging task of distribution aligning EEG data, however, if achieved offers the possibility to learn generalized emotion classifier models independent of hardware and experimental design. Additionally, private encoded representations offer BCI researchers to publish useful non-identifiable EEG extracts without granting full access to the dataset and thereby enable researchers to exchange EEG experimental data more effectively. 

%3. How we solved the problem?
In this work we propose a multi-source learning framework, consisting of one shared classifier and multiple private encoders, regularized by a MMD-based domain-alignment loss. Using a non-trainable classifier we show, that we are successfully decreasing the domain-covariance of the learned representations. We evaluate our framework using EEG datasets with emotional label and compare our classification results against a encoder-classifier-model that was learned and tested on each dataset individually. 

%4. How do we know the problem was (still needs to be) solved?
We show, that multi-source learning is a promising approach for learning domain invariant representations. However, this new field of research poses significant challenges, for example as the gap of the domain-alignment-loss between training and validation can not be explained by the state-of-the-art. In addition we show that Batchnormalization layers as well as Dropout layers seem to have yet unknown impact on the training of multi-source setups.


%contribution statement:
\subsection{Contribution Statement}
Our paper makes the following contributions:
\begin{itemize}
    \item proposition of learning framework and preprocessing steps for data-source-invariant representation learning for EEG data
    \item analysis of data-source domain invariance on multiple emotional EEG datasets
    \item definition of obstacles and solutions for achieving domain invariance in EEG data
\end{itemize}
We show that, DAPE learns EEG representations, that can predict emotions with reasonable accuracy of $50\%$ in effect $2\%$ lower than traditional baseline approaches across 4 different data source domains, while also reducing privacy leaking information of $-40\%$ (domain classifier). Thereby demonstrating the usefulness of regularizing the domain-leakage information in future EEG encoding applications while achieving similar classification accuracies.


%\clearpage

%potential points made by reviewers:
%1. why is overall emotion detection accuracy so little in comparison to RW?
\begin{figure}[h]
    \centering
    \includegraphics[]{images/DAPE_baseline_comparison.eps}
    \caption{Comparison of the multi-source learning Framework with a single-source baseline model}
    \label{fig:my_label}
\end{figure}
%2.what are general methods for achieving domain invariance? How can we be sure to trust that MMD regularization is the right way -> check RW
%3.why do we need multi-source learning at all? 
%4. Why would I need a representation when doing multi-source learning?
